Two c's in a pod: Cosmology independent measurement of the Type Ia supernova colour-luminosity relation with a sibling pair

Using Zwicky Transient Facility (ZTF) observations, we identify a pair of "sibling" Type Ia supernovae (SNe Ia), i.e., hosted by the same galaxy at z = 0.0541. They exploded within 200 days from each other at a separation of $0.6^{"} $ corresponding to a projected distance of only 0.6 kpc. Performing SALT2 light curve fits to the gri ZTF photometry, we show that for these equally distant "standardizable candles", there is a difference of 2 magnitudes in their rest frame B-band peaks, and the fainter SN has a significantly red SALT2 colour $c = 0.57 \pm$ 0.04, while the stretch values $x_1$ of the two SNe are similar, suggesting that the fainter SN is attenuated by dust in the interstellar medium of the host galaxy. We use these measurements to infer the SALT2 colour standardization parameter, $\beta$ = 3.5 $\pm$ 0.3, independent of the underlying cosmology and Malmquist bias. Assuming the colour excess is entirely due to dust, the result differs by $2\sigma$ from the average Milky-Way total-to-selective extinction ratio, but is in good agreement with the colour-brightness corrections empirically derived from the most recent SN Ia Hubble-Lemaitre diagram fits. Thus we suggest that SN "siblings", which will increasingly be discovered in the coming years, can be used to probe the validity of the colour and lightcurve shape corrections using in SN Ia cosmology while avoiding important systematic effects in their inference from global multi-parameter fits to inhomogeneous data-sets, and also help constrain the role of interstellar dust in SN Ia cosmology.

==> galaxy_sed.tex <==
We retrieved science-ready coadded images from the Sloan Digital Sky Survey data release 9 (SDSS DR 9; \citealt{Ahn2012a}), the Panoramic Survey Telescope and Rapid Response System (Pan-STARRS, PS1) DR1 \citep{Chambers2016a}, the Two Micron All Sky Survey \citep[2MASS;][]{Skrutskie2006a}, and preprocessed \wise\ images \citep{Wright2010a} from the unWISE archive \citep{Lang2014a}\footnote{\href{http://unwise.me}{http://unwise.me}}. The unWISE images are based on the public \wise\ data and include images from the ongoing NEOWISE-Reactivation mission R3 \citep{Mainzer2014a, Meisner2017a}.

We used the software package LAMBDAR (Lambda Adaptive Multi-Band Deblending Algorithm in R) \citep{Wright2016a}, which is based on a software package written by \citet{Bourne2012a} and tools presented in \citet{Schulze2020a}, to measure the brightness of the host galaxy. The spectral energy distribution was modelled with the spectral energy distributions (SEDs) with the software package \package{Prospector}\footnote{\href{https://github.com/bd-j/prospector}{https://github.com/bd-j/prospector}} version 0.3 \citep{Leja2017a}. We assumed a linear-exponential star-formation history, the \citet{Chabrier2003a} IMF, the \citet{Calzetti2000a} attenuation model, and the \citet{Byler2017a} model for the ionized gas contribution. The priors were set as described in \citet{Schulze2020a}.


==> introduction.tex <==
\section{Introduction}
\label{sec:intro}
Perhaps we will need to discuss the \LCDM\ model and cite ~\citet{2019ApJ...873..111I} or will depend on something in~\citep{2009arXiv0912.0201L}.

\begin{figure}[!htp]
    \begin{center}
    \includegraphics[width=0.45\textwidth]{./test_fig}
        \caption{Test figure: The purpose is simply to check that the caption and figure number work correctly.
    \label{fig:test_fig}
        }
    \end{center}
\end{figure}



==> journaldefs.tex <==
\newcommand{\aap}{Astron.\ Astrophys.}
%\newcommand{\apj}{ApJ}
\newcommand{\apjl}{Astrophys.J.Lett.\ }
%\newcommand{\prd}{Phys.Rev.D.}
\newcommand{\mnras}{MNRAS}
\newcommand{\jcap}{JCAP}
%\newcommand{\nat}{Nature}
\newcommand{\physrep}{Physics Reports}
\newcommand{\pasp}{PASP}
\newcommand{\aaps}{Astron.\ Astrophys.\ Suppl.\ Ser.\ }
\newcommand{\aj}{Astron.\ J.\ }


==> peakmags_app.tex <==
\begin{table*}
\caption{Peak synthetic magnitudes in ZTF bands and the rest frame Bessell B band from the best fit \salt\ models for \oldsn\ and \newsn\ }
\begin{tabular}{ccccc}
id & ztfg (mags) & ztfr (mags) & ztfi (mags) & Bessell B (mags) \\
\oldsn\ & 19.4 & 18.8 & 19.1 & 19.7 \\
\newsn\ & 17.5 & 17.6 & 18.2 & 17.6 \\
\end{tabular}
\label{tab:app_peakmags}
\end{table*}

